Identifying Non-Control Security-Critical Data through Program Dependence Learning

As control-flow protection gets widely deployed, it is difficult for attackers to corrupt control-data and achieve control-flow hijacking. Instead, data-oriented attacks, which manipulate non-control data, have been demonstrated to be feasible and powerful. In data-oriented attacks, a fundamental step is to identify non-control, security-critical data. However, critical data identification processes are not scalable in previous works, because they mainly rely on tedious human efforts to identify critical data. To address this issue, we propose a novel approach that combines traditional program analysis with deep learning. At a higher level, by examining how analysts identify critical data, we first propose dynamic analysis algorithms to identify the program semantics (and features) that are correlated with the impact of a critical data. Then, motivated by the unique challenges in the critical data identification task, we formalize the distinguishing features and use customized program dependence graphs (PDG) to embed the features. Different from previous works using deep learning to learn basic program semantics, this paper adopts a special neural network architecture that can capture the long dependency paths (in the PDG), through which a critical variable propagates its impact. We have implemented a fully-automatic toolchain and conducted comprehensive evaluations. According to the evaluations, our model can achieve 90% accuracy. The toolchain uncovers 80 potential critical variables in Google FuzzBench. In addition, we demonstrate the harmfulness of the exploits using the identified critical variables by simulating 7 data-oriented attacks through GDB.

==> Makefile <==
PAPER = main
REFERENCE = main
JUNK =*.log *.synctex\(busy\) *.xml *.bcf *.toc *.snm *.nav *.fls *.fdb_latexmk *.synctex.gz *.spl *.ps *.dvi  *.out *.aux *.backup *~ *.blg
COUNTING_TOOL = ./texcount.pl
TEMP = 0
MY_VAR=$(shell echo whatever)

# Define the tools we are going to use

all: pdf

# Rules for various parts of the target
pdf: $(PAPER).tex
	pdflatex $(PAPER).tex
	bibtex $(PAPER).aux
	pdflatex $(PAPER).tex
	pdflatex $(PAPER).tex
	#rm -f $(JUNK)

clean:
	rm -f $(JUNK) $(PAPER).pdf




==> anotheridea.tex <==
The limitation of source code representation

1. The meaning of variable name.
2. Learning from 


Source code learning cannot achieve good results.


==> bitcode.tex <==
\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{mygray}{gray}{0.9}
\lstset{
language=C,
frame=tb,
basicstyle={\footnotesize \bf \ttfamily}, %\scriptsize,\ttfamily,%
tabsize=3,
breaklines=true,
% breakatwhitespace=false,
showstringspaces=false,
% columns=fullflexible,
numbers=left,
numbersep=-10pt,                     % where to put the line-numbers
escapeinside={(*}{*)},
xleftmargin=2pt,
numberstyle=\texttt \footnotesize,% \scriptsize %\tiny, %\,
stringstyle=\color{mauve},
keywordstyle= \color{black}, % \color{blue},
commentstyle=\color{dkgreen} \textit,%\scriptsize \textit,
}
\begin{figure}[h] 
%\vspace{-1.6ex}
% \setlength{\belowcaptionskip}{-13pt}
% \setlength{\abovecaptionskip}{-13pt}
\begin{lstlisting}[language=C++,
    directivestyle={\color{black}}
    emph={int,char,double,float,unsigned},
    emphstyle={\color{blue}},caption={A piece of code with critical data.},label=code:bit,captionpos=b]
    uint8_t user_bits = 0;
    void do_authentication(char *user, ...) {
        ...
        while (user_bits & AUTH_MASK) {
        /* Get a packet from the client */
        type = packet_read();
        switch (type) {
            ...
            case SSH_CMSG_AUTH_PASSWORD:
                if (auth_password(user, password))
                    authenticated |= AUTH_MASK;
            case ...
        }
        if (user_bits & AUTH_MASK) break;
    }
    /* Perform session preparation. */
    do_authenticated(pw);
\end{lstlisting}
%\vspace{-3.5ex}
\end{figure} 


==> casestudy.tex <==

\subsection{Case study}
\label{sec:case}

In this section, we conduct case studies to provide our insights about the model decisions. Note that all the statements made in this section are not general conclusions. 


%\subsection{True Positive and True Negative Cases}

\mypara{True Positive}
%
We first start with the model's successes. 
Our model correctly classified the examples shown in the introduction as positive examples. 
As explained in the introduction section, variable {\tt aclp} will carry the information about whether the user is blocked, 
and an attacker can illegally login if the value of the variable is modified during the execution. 
The dependence tree contains the information of the critical operation shown in Code 2, 
and our trained model is able to capture that information. 
% (\hypertarget{evidence1}{\hyperlink{observation1}{\textbf{E1}}}:) 
% Note that the \autoref{fig:dfg-tree} does not show the complete long dependence tree, which contains a good amount of information. 
For example, the opcode feature shows that there are several data transfer operations (\cc{MOV} instructions) and several logical operations. 
% Although not shown in the \autoref{fig:dfg-tree}, 
% there is also a vector operation opcode. 
The number of dominated BBs is also fairly big, which results in 67 changed executed BBs. 
Though it is not possible to completely explain a deep learning model's decision, 
it is clear that the information is rich in this example, and heuristically, 
a variable that is processed by diverse opcodes and with many control dependencies is likely to be critical. 
% \zl{more specific. We can talk about the 1) mov instruction. We can talk about 2) logical operation, 3) bb\_diff, 4) fake the bb\_diff and see the result. } 

% \begin{figure}[!htbp]
%   % \setlength{\belowcaptionskip}{-13pt}
%   \centering
%   \includegraphics[width=0.45\textwidth]{graphs/proftpd14_3.png}
%   \caption{The Structure of the Data Flow Tree of \autoref{code:bit}.}
%   \label{fig:cs_tp}
% \end{figure}

\mypara{True Negative}
%
We also discuss an example that the model correctly identifies non-critical data.
The variable \cc{daemonmode} in {\tt bftpd-5.6} controls 
whether the server should be run as a daemon or not.
% which is very unlikely to be interested by an attacker. 
% Even if an attacker manages to modify it, 
% the server maintainer will immediately realize that the program is not running as expected. 
With careful checks, 
we believe this variable is non-critical
as the program behavior is almost the same
regardless whether the program is running as daemon or not.
The use of this variable is quite simple: 
it is initialized with a value from the command line 
or the configuration file, and 
then gets checked during the program setup
before spawning the daemon. 
These uses result in three dependence trees are partially shown in \autoref{fig:cs_abs} (a). 
The dependency paths in these tree are short and no fork is presented. 
% Although one can observe the CMP operations, 
% it is not likely a critical variable to have such short data flow. 
% For example, 
% an authentication flag will have a more complicated data flow, 
% as the program will need to check many conditions. 
In addition, the number of dominated BBs is only 1, 
which means that the only few basic block control dependent on it.
% executed basic blocks are only changed by 1
% when it is flipped.
%
% We believe this is the main reason that
% our model classifies this variable as non-critical.
% \haizhou{For every case, we mention 4 things: 1) straight lines, 2) logical operation, 3) bb\_diff, 4) not very long (simple dfg)}

% \begin{figure}[!htbp]
%   % \setlength{\belowcaptionskip}{-13pt}
%   \centering
%   \includegraphics[width=0.45\textwidth]{graphs/bftpd_36.png}
%   \caption{The Data Flow Tree of Variable {\tt daemonmode}.}
%   \label{fig:cs_tn}
% \end{figure}


%% Next, we take a close look at the model's failures: another two examples from {\tt bftpd-5.6}. 


\begin{figure}[t]
  % \setlength{\belowcaptionskip}{-13pt}
  \centering
  \includegraphics[width=0.38\textwidth]{graphs/casestudy.pdf}
  \caption{\textbf{Dependence subtrees for case studies.}}
  \label{fig:cs_abs}
\end{figure}


\mypara{False Positive} 
%
In this example, our model incorrectly classifies one non-critical variable as critical.
Specifically, variable {\tt local} is used in \cc{bftpd-5.6} to 
find the timezone difference between a client and the server, 
only for security-unrelated operations such as logging.
But our model gives the unexpected label. 
By checking its dependence trees partially shown in \autoref{fig:cs_abs} (b), 
we found that the dependencies are complicated,
including many comparison and logical operations to compare two time zones,
% as finding a time zone difference involves many comparisons. 
%%Further more, there are many branches in the data-flow tree, 
%which implies the value of the variable is not acquire in a straight forward manner. 
%This observation is usually related to the critical flags. 
The number of dominated BBs is 5, 
indicating this variable can slightly influence 
the overall program execution. 
All these facts confuse our model to draw 
the wrong conclusion. 
%
A human analyst can filter this variable out 
when figuring out that it is not related to security-related operations. 
However, at binary level no comment or name information in the traces can be used.
%the model does not have access to this important information. 
% Therefore, in this case the model does not have sufficient information, 
% and thus treats the dependencies of a non-critical variable 
% as one of critical variables. 
% \haizhou{ 1) fairly long, 2) logical operation, 3) bb\_diff, 4) high level semantics: be specific; 5) high level semantics not captured}


% \begin{figure}[h] 
% \vspace{-1.6ex}
% % \setlength{\belowcaptionskip}{-13pt}
% % \setlength{\abovecaptionskip}{-13pt}
% \begin{lstlisting}[language=C++,
%     directivestyle={\color{black}},
%     emph={int,char,double,float,unsigned, static, const, if, return, goto},
%     emphstyle={\color{blue}},caption={Example of Misclassified Non-Critical Data},label=code:cs_fp,captionpos=b]
%     int Get_Time_Zone_Difference()
%     {
%       ...
%       /* grab current time */
%       local_time = localtime( &my_time );
%       memcpy(&local, local_time, sizeof(struct tm) );

%       /* find time zone difference */
%       ...
%     }
% \end{lstlisting}
% \vspace{-3.5ex}
% \end{figure} 

% \begin{figure}[!htbp]
%   % \setlength{\belowcaptionskip}{-13pt}
%   \centering
%   \includegraphics[width=0.45\textwidth]{graphs/bftpd_25.png}
%   \caption{The Data Flow Tree of Variable {\tt local}.}
%   \label{fig:cs_fp}
% \end{figure}

% Lastly, we examine a case when the model misclassify a positive example. The variable is called {\tt anon\_ok}, which is a flag to indicate whether the anonymous logins are allowed. By modifying this flag, the attacker can anonymously login to the server with the anonymous login is being disabled in the configuration. Anonymous login has risks of illegal usage and deny-of-service attacks, so many administrators will disable this functionality. Therefore, this variable is considered as critical. In \autoref{fig:cs_abs} (c), a define data flow subtree and a use data flow subtree is shown. In the define tree, there is a vector operation, which is mainly for parallel numerical calculation. In the use tree, although there is a CMP operation, but the data flow is short and straight forward. From the dataflow, one may guess that this is a non-critical data that is calculated through some intense calculation, and then used as a flag. Especially when the global control-dependency is 17, which is a small number, and there is no logical operations. In general, one of the few case this data could be critical is encryption related data, but encryption related data usually has very rich dataflow pattern, and the model do not think this is the case. Therefore, the model classify this data as non-critical.

\mypara{False Negative}
%
Lastly, we examine a case where the model misses a critical variable. 
{\tt anon\_ok} is a flag indicating whether anonymous logins are allowed. 
By modifying this flag, attackers can anonymously login to the server,
and then conduct illegal access or launch deny-of-service attacks.
%so many administrators will disable this functionality. 
% Therefore, this variable should be considered as critical. 
\autoref{fig:cs_abs} (c) shows its full define-flow tree (left) and use-flow tree (right).
The define-flow tree has a vector operation,
and the use-flow tree contains a \cc{CMP} operation.
The whole paths of dependencies are fairly short,
and the number of dominated BBs is only 17, which could indicate that 
this variable is not very critical. 
%This data could be critical 
%when it is encryption-related data, 
%but encryption-related data usually has unique data-flow pattern, 
%and the model does not think this is the case. 
%
The reason for this misclassification is similar to the false positive case. 
When a human analyst looks at the variable, 
it is obvious that the data is related to anonymous login and thus critical,
but the model does not have access to this information.
% However, the model does not have access to this information at binary level, and if the dependence graph appears to not contain conspicuous features that are relevant to critical data, the model is possible to have a misclassification. 
% \haizhou{ 1) fairly short, 2) minimal logical operation, 3) bb\_diff, 4) high level semantics: be specific; 5) high level semantics not captured}

% \zl{Admit that a our mulatation strategy is not robust in all case, which could be a reason of false negative.}

% From the 4 examples, we have following observations:
% \begin{itemize}
%     \item The model tends to classify a data with long data flow and complicated branches in the data flow tree as critical data. Especially when the global dependency is high and there are fair amount of logical operations.
%     \item The model tends to classify a data with very short data flow with minimal number of branches in the data flow tree as non-critical.
%     \item The model perform worse when important information cannot be provided at binary level.
% \end{itemize}
% Further more, when we find global dependencies, our mutation strategy is not robust in all cases, which can cause inconsistency of this feature and thus performance deterioration.

% \begin{figure}[h] 
% \vspace{-1.6ex}
% % \setlength{\belowcaptionskip}{-13pt}
% % \setlength{\abovecaptionskip}{-13pt}
% \begin{lstlisting}[language=C++,
%     directivestyle={\color{black}},
%     emph={int,char,double,float,unsigned, static, const, if, return, goto},
%     emphstyle={\color{blue}},caption={Example of Misclassified Critical Data},label=code:cs_fn,captionpos=b]
%     int bftpd_login(char *password)
%     {
%         ...
%         int anon_ok = FALSE;
%         ...
%         if (! strcasecmp(anonymous, "yes") )
%     	   anon_ok = TRUE;
%     	...
%     	if ( anon_ok && ! change_uid )
%         ...
%     }
% \end{lstlisting}
% \vspace{-3.5ex}
% \end{figure} 

% \begin{figure}[!htbp]
%   % \setlength{\belowcaptionskip}{-13pt}
%   \centering
%   \includegraphics[width=0.45\textwidth]{graphs/bftpd_29.png}
%   \caption{The Structure of the Data Flow Tree of Variable {\tt anon\_ok}.}
%   \label{fig:cs_fn}
% \end{figure}






==> dataflowcode.tex <==
\begin{figure}[h] 
%\vspace{-1.6ex}
% \setlength{\belowcaptionskip}{-13pt}
% \setlength{\abovecaptionskip}{-13pt}
\begin{lstlisting}[language=C,
    %emph={int,char,double,float,unsigned},
    emphstyle={\color{blue}},caption={\textbf{Operations on critical data \cc{aclp} in \cc{proftpd}}.},label=code:df,captionpos=b]
    res = (res || rres);
    aclp = res; //value passed through function return
    if (c == NULL && aclp == 0){ ... }
\end{lstlisting}
%\vspace{-3.5ex}
\end{figure} 


==> defination.tex <==
\zl{Can we give a formal defination of critical data?}

==> experiment.tex <==



==> graphs/overfig.tex <==

% \subimport{./layers/}{init}


\def\ConvColor{rgb:yellow,5;red,2.5;white,5}
\def\ConvReluColor{rgb:yellow,5;red,5;white,5}
\def\PoolColor{rgb:red,1;black,0.3}
\def\DcnvColor{rgb:blue,5;green,2.5;white,5}
\def\SoftmaxColor{rgb:magenta,5;black,7}
\def\SumColor{rgb:blue,5;green,15}

\begin{figure*}
\begin{tikzpicture}
\tikzstyle{connection}=[ultra thick,every node/.style={sloped,allow upside down},draw=\edgecolor,opacity=0.7]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Draw Layer Blocks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[canvas is zy plane at x=0, name=code] (temp) at (-4,0,0) {\includegraphics[width=8cm,height=8cm]{graphs/code.png}};
\node[name=codecap] (temp) at (-4,-5,0) {code};


% conv1_1,conv1_2,%pool1
% \pic[shift={(0,0,0)}] at (0,0,0) {\includegraphics[width=8cm,height=8cm]{cats.jpg}};
\node[canvas is zy plane at x=0, name=pgraph] (temp) at (0,0,0) {\includegraphics[width=10cm,height=10cm]{graphs/pdg.png}};
\node[name=codecap] (temp) at (0,-5,0) {PDG};
\draw [connection]  (-3,0,0)    -- node {\midarrow} (-1,0,0);

\node[canvas is zy plane at x=0, name=tree] (temp) at (3,0,0) {\includegraphics[width=7cm,height=7cm]{graphs/tree.png}};
\node[name=codecap] (temp) at (3,-3,0) {sub-PDG};

\draw [connection]  (0,0,0)    -- node {\midarrow} (3,0,0);

\pic[shift={(0,2,0)}] at (6,-2.8,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=16}};
\pic[shift={(0,2,0)}] at (6,-1.4,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=16}};
\pic[shift={(0,2,0)}] at (6,0,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=16}};
\pic[shift={(0,2,0)}] at (6,1.4,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=16}};
\pic[shift={(0,2,0)}] at (6,2.8,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=16}};

\node[canvas is zy plane at x=0, name=gstructure] (temp) at (6,-5.5,0) {\includegraphics[width=6cm,height=6cm]{graphs/gstructure.png}};
\node[name=codecap] (temp) at (6,-8.5,0) {graph structure};

\node[name=nodefeat] (temp) at (6,-2.5,0) {node features};
\draw [connection]  (3.5,0,0)    -- node {\midarrow} (5.5,0,0);

\draw [connection]  (3,-1,0)    -- node {\midarrow} (3,-5.5,0);
\draw [connection]  (3,-5.5,0)    -- node {\midarrow} (5.5,-5.5,0);

\node[name=gnn] (temp) at (9,0,0) {\includegraphics[width=2cm,height=8cm]{graphs/gnnlayer1.png}};
\node[name=codecap] (temp) at (10,-5,0) {layer 1};
\draw [connection]  (6.5,0,0)    -- node {\midarrow} (8.5,0,0);

\draw [connection]  (6.5,-5.5,0)    -- node {\midarrow} (9,-5.5,0);
\draw [connection]  (9,-5.5,0)    -- node {\midarrow} (9,-1,0);



\pic[shift={(0,0,0)}] at (12,-2.4,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=14}};
\pic[shift={(0,0,0)}] at (12,-1.2,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=14}};
\pic[shift={(0,0,0)}] at (12,0,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=14}};
\pic[shift={(0,0,0)}] at (12,1.2,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=14}};
\pic[shift={(0,0,0)}] at (12,2.4,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=14}};

\node[name=noderepresentation] (temp) at (12,-6,0) {node representation};
\draw [connection]  (9.5,0,0)    -- node {\midarrow} (11.5,0,0);


\node[name=gnn] (temp) at (15,0,0) {\includegraphics[width=1.6cm,height=7cm]{graphs/gnnlayer2.png}};
\node[name=codecap] (temp) at (15,-5,0) {layer 2};
\draw [connection]  (12.5,0,0)    -- node {\midarrow} (14.5,0,0);

\draw [connection]  (9,-5.5,0)    -- node {\midarrow} (15,-5.5,0);
\draw [connection]  (15,-5.5,0)    -- node {\midarrow} (15,-1,0);

\pic[shift={(0,0,0)}] at (18,-2.4,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=12}};
\pic[shift={(0,0,0)}] at (18,-1.2,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=12}};
\pic[shift={(0,0,0)}] at (18,0,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=12}};
\pic[shift={(0,0,0)}] at (18,1.2,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=12}};
\pic[shift={(0,0,0)}] at (18,2.4,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=12}};

\node[name=noderepresentation] (temp) at (18,-6,0) {node representation};
\draw [connection]  (15.5,0,0)    -- node {\midarrow} (17.5,0,0);



\node[name=gnn] (temp) at (21,0,0) {\includegraphics[width=1.4cm,height=6cm]{graphs/gnnlayer3.png}};
\node[name=codecap] (temp) at (21,-5,0) {layer 3};
\draw [connection]  (18.5,0,0)    -- node {\midarrow} (20.5,0,0);

\draw [connection]  (15,-5.5,0)    -- node {\midarrow} (21,-5.5,0);
\draw [connection]  (21,-5.5,0)    -- node {\midarrow} (21,-1,0);

\pic[shift={(0,0,0)}] at (24,-2.4,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=10}};
\pic[shift={(0,0,0)}] at (23,-1.2,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=10}};
\pic[shift={(0,0,0)}] at (24,0,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=10}};
\pic[shift={(0,0,0)}] at (24,1.2,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=10}};
\pic[shift={(0,0,0)}] at (24,2.4,0) {RightBandedBox={name=cr2,%
        zlabel={{64}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width=1.5,depth=10}};

\node[name=noderepresentation] (temp) at (24,-6,0) {node representation};
\draw [connection]  (21.5,0,0)    -- node {\midarrow} (23.5,0,0);

\pic[shift={(0,0,0)}] at (27,0,0) {RightBandedBox={name=cr2,%
        zlabel={{8}},fill=\ConvColor,bandfill=\ConvReluColor,%
        height=1.5,width={1.5},depth=10}};
\node[name=graphrepresentation] (temp) at (27,-3,0) {graph representation};
\draw [connection]  (24.5,0,0)    -- node {\midarrow} (26.5,0,0);

\pic[shift={(0,0,0)}] at (30,0,0) {Ball={name=elt1,%
        fill=\SumColor,opacity=0.6,%
        radius=2.5,logo=$$}};
\node[name=graphrepresentation] (temp) at (30,-2,0) {output layer};
\draw [connection]  (27.5,0,0)    -- node {\midarrow} (29.5,0,0);

\node[name=graphrepresentation] (temp) at (33,0,0) {output};
\draw [connection]  (30.5,0,0)    -- node {\midarrow} (32.5,0,0);

\end{tikzpicture}
\end{figure*}


==> idea.tex <==
Variable centric learning tasks.

We have a new insight - In theory, there is a space of such learning task, however, not every learning task in this 
learning space can be full-filled through dataflow analysis.

In this work, we focus on the subspace, where dataflow analysis is essential. We believe 
this subspace is one of the most interesting and one of the most important, especially 
in the perspective of software security, realizability, and safety.
In this way, we can explain we focus on this field.

Based on the new insight, we have the following hypnosis:

\textbf{H1:} This purpose deep learning based, dataflow analysis oriented representation could be learned to deal with important subspace.
In this work, we are going to learn such general purpose representation, then, we are going to use several variable centric learning tasks (loop control variable, critical data, variable type classification).

The main challenges: 
\textit{Challenge 1:} Stand dfg would fail to get good results.
\textit{Challenge 2:} GNN and RGCN is not scalable.

Currently, 
1. People have no agreement regarding the appropriate neural network architecture.
2. People have no agreement regarding the preprocessing.

So, some research is needed.

insight1: our key idea is Tree-LSTM could be scalable and accurate simultaneously.

insight2: dataflow analysis can capture the essential XY relationship, that are cross-task useful. 
e.g., in critical data identification,
    - X is variable, 
    - Y is how variable is defined and used.
another example:
    - X is variable,
    - Y is another variable tainted by X.

Given DFG+, we should be able get a set of XY relationships. The set of XY in CCS submission is not suitable for cross task.

We observe two requirement for set of XY relationship for cross task:
1. keep as many XY as possible for one variable (for example, the taint propagation should not cut too short).
2. Enough training sample.
3. General learning task.










==> implementation.tex <==
\section{Implementation}

We implemented the Tree-LSTM learning 
algorithm based on the implementation in \cite{XXX}. 
We implemented the baseline RGCN learning algorithm based on the deep graph library
(DGL)~\cite{wang2019dgl}. 
%and train the model using  with different number of layers  

==> layers/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}



==> longtable.tex <==
% \begin{table}[htp]
    \onecolumn
\scriptsize
\begin{ThreePartTable}
\begin{TableNotes}
    \item [1] Deep Learning metrics are often not available in fuzzing papers. Typical fuzzing metrics used for evaluations are: code coverage, pass rate and bugs.
    %\item [2] 
\end{TableNotes}
\begin{longtable}{p{1.4cm}<{\centering}p{1.4cm}<{\centering}cccccc}
\captionsetup{width=.95\textwidth}
\caption{\footnotesize Solutions using Deep Learning for eight security problems. The metrics in the Evaluation column include accuracy (ACC), precision (PRC), recall (REC), $F_{1}$ score ($F_{1}$), false positive rate (FPR), and false negative rate (FNR).}
\label{Table:Summary}\\

\toprule \toprule
\textbf{Security Problem} & \textbf{Works} & \multicolumn{6}{c}{\textbf{Summary}} \\
\cmidrule[1pt]{1-8}
\endfirsthead




% \hline\hline
\insertTableNotes 
\endlastfoot

    

    \bottomrule
    \bottomrule
    % \end{table}
    \end{longtable}
    \begin{TableNotes}
        \item [1] Deep Learning metrics are often not available in fuzzing papers. Typical fuzzing metrics used for evaluations are: code coverage, pass rate and bugs.
    \end{TableNotes}
\end{ThreePartTable}


